Difference-in-Differences: Bridging Normalization and Disentanglement in PG-GAN

What mechanisms causes GAN's entanglement? Although developing disentangled GAN has attracted sufficient attention, it is unclear how entanglement is originated by GAN transformation. We in this research propose a difference-in-difference (DID) counterfactual framework to design experiments for analyzing the entanglement mechanism in on of the Progressive-growing GAN (PG-GAN). Our experiment clarify the mechanisms how pixel normalization causes PG-GAN entanglement during a input-unit-ablation transformation. We discover that pixel normalization causes object entanglement by in-painting the area occupied by ablated objects. We also discover the unit-object relation determines whether and how pixel normalization causes objects entanglement. Our DID framework theoretically guarantees that the mechanisms that we discover is solid, explainable and comprehensively.

==> 4-preservation.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{1.7in}
    \includegraphics[width=1.7in]{figures/66-ablate-chair2.PNG}
    \caption{}
    \end{subfigure}
    \begin{subfigure}[t]{1.7in}
    \includegraphics[width=1.7in]{figures/1-ablate_chair.PNG}
    \caption{}
    \end{subfigure}
    \begin{subfigure}[t]{1.7in}
    \includegraphics[width=1.7in]{figures/122-ablate-chair.PNG}
    \caption{}
    \end{subfigure}
    \caption{Ablating top-20 chair-ACE units, chairs only shrink slightly or change their color. It's very hard to entirely remove them.}
    \label{ablate_chair}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{1.8in}
    \includegraphics[width=2.0in]{figures/seg_ablate20.png}
    \caption{}
    \label{fig:segarea_ablate20_variousobjects}
    \end{subfigure}
    \begin{subfigure}[t]{1.8in}
    \includegraphics[width=2.0in]{figures/chair_sc_fix_beta.png}
    \caption{}
    \label{fig:segarea_ablate20_fix}
    \end{subfigure}
    \begin{subfigure}[t]{1.8in}
    \includegraphics[width=2.0in]{figures/distplot.png}
    \caption{}
    \label{fig:ace-distribution}
    \end{subfigure}
    \caption{(a) To remove a kind of object, we can usually get good result by ablating top-20 units with highest ACE for this objects (e.g. painting, window, light, curtain and person); However, ablating top-20 chair-ACE units only results in a drop of $20\%$ on chairs' area, and we need to ablate at least top-80 chair-ACE units to get a noticeable effect. (b) After fixing $\beta$, the drop of chair area is almost proportional to the number of ablated units, which is much better than the case not fix $\beta$. (c) The distribution of units from layer 4 over chair-ACE and painting-ACE. A unit is counted if it has ACE $\geq$ 0.15, since we focus on the units with observable effect on chair or painting. Since the units with ACE $\geq$ 0.6 all have great impact on the corresponding object class but are relatively few and distributed, we treat them as units with ACE $=$ 0.6.}
\end{figure}
\begin{figure}[htbp]
    \begin{center}
    \begin{subfigure}[t]{0.9in}
    \includegraphics[width=0.9in]{figures/1-original.png}
    \caption{original}
    \end{subfigure}
    \begin{subfigure}[t]{1.0in}
    \includegraphics[width=1.0in]{figures/yminusybar.png}
    \caption{$Y-\overline{Y}$}
    \end{subfigure}
    \begin{subfigure}[t]{1.0in}
    \includegraphics[width=1.0in]{figures/yuminusyprime.png}
    \caption{$\underline{Y}-Y'$}
    \end{subfigure}
    \begin{subfigure}[t]{1.0in}
    \includegraphics[width=1.0in]{figures/diff-in-diff.png}
    \caption{$(Y-\overline{Y})-(\underline{Y}-Y')$}
    \end{subfigure}
    \end{center}
    \caption{The heatmap of difference-in-difference experimental results. We first calculate the difference of corresponding output tensors and then plot the heatmap of the length of the vector(R,G,B). }
    \label{diff-in-diff}
\end{figure}
\section{Preservation: Entanglement on unsuppressbile objects}
In this section, we will discuss the first type of entangled phenomenon: deactivating-ablation entanglement. Compared to \xiao{} in Figure , in Figure \ref{ablate_chair}, ablating units related to chairs with top ACE effects can not remove or eliminate chairs, only causing them to reduce sizes and density, or change color. In literature, researchers conduct a number of experiments and qualitatively exhibit that the ease of removing a class of objects varies with the scene type, such as windows in bedroom are as hard as chairs in conference room to be removed~(\cite{bau2018gan}), which implies that GAN has learned some scene-specific knowledge. 

Our quantitative experiments also support the conclusion (see Figure \ref{fig:segarea_ablate20_variousobjects}). Given an object class (such as chair or painting), we rank units by its causal contributions from strong to weak, and sequentially ablate them to observe a decline in area of the object class. As the diagram demonstrated, there is an apparent contrast between chair and others, showing the existence of a strong entanglement between chair objects and the environment. 

However, this entanglement is substantially diminished when we fix the normalizing coefficients $\beta$ as shown in Figure \ref{fig:segarea_ablate20_fix}, in which the pixel normalization $N$ should be playing a critical role. 

To some extend, this difference could be explained by the distribution of units according to ACE (Figure \ref{fig:ace-distribution}), where units of removable class almost locate at high-ACE but unsuppressible ones lie at low-ACE.



==> 5-substitution.tex <==
\section{Substitution: Entanglement on emerged object}
This section focus on another strange phenomenon: although we can successfully remove an object that is not so important in the scenario by ablating several top-ACE related units, sometime there will be some other strange objects appear. For example, in Figure. \ref{33-seg}, after we ablate top-20 painting-ACE units, paintings are totally disappear. However, some door-like things appear on the wall while what we expect to see is that we can get clean wall after removing these paintings. 

To explain why other things will appear after removing painting, we first do semantic segmentation on the image after ablating top-20 painting-ACE units. (Figure. \ref{33-seg}) using the same segmenter as in GAN Dissecion. The result shows that things that come up are some mixture of window, door, cabinet and fabric similar to curtain.
\begin{figure}[htbp]
    \begin{center}
    \includegraphics[width=4in]{figures/33-seg-compare.PNG}
    \caption{After ablating top-20 painting-ACE units in layer 4, the painting totally disappear, but there are some other door-like objects appear. The segmenter thinks the things that come up are some mixture of window, door, cabinet and fabric like curtain.}
    \label{33-seg}
    \end{center}
\end{figure}

Above phenomenon shows that although painting has highly concentrated ACE distribution, it  may be not totally disentangled with other objects thus they would appear after it is removed. And except painting-ACE units, there must be plenty of units in the same layer that have ACE for the objects that emerges on the wall, but their effect are covered up by painting-ACE units so only if we ablating top painting-ACE units and under the enhancement caused by pixel normalization, can these units' effect be represented. 

Based on this idea, we choose several objects that might appear on the wall and then get top-50 units in layer 4 that have the max activation value on the point door appears (Figure \ref{33-ranking}). We calculate and normalize the sum of these units' ACE for each particular object. We find that before ablation, the ACE for painting is the largest and there are also large ACE for window, curtain, and door, which implies that they are very likely to appear after removing paintings. As expected, after ablating top-20 painting-ACE units, ACE for curtain, door and window becomes the largest three and curtain-like fabric, door and window indeed appear at this point. Moreover, these remain units' absolute activation value at this point increases by about 9\% because of pixel normalization, which helps the appearance of fabric and door. This shows that GANs generate images by stacking many different features but may only show the most activated feature at last. If we remove some objects with high degree of disentangle, other objects with relatively smaller activated value may appear, and further fill the image under the enhancement of pixel normalization. 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=5.0in]{figures/33-rank-change.PNG}

    \caption{We choose top-50 units with max activation on the point where door appears (red point) and calculate and normalize their ACE for different objects that are likely appear on the wall. Before ablation, ACE for painting is the largest ACE-related units, but ACE for window, curtain and door are also quite large. After ablation, the decrease of painting ACE and increase of wall ACE also make painting removed and replaced with wall. Moreover, ACE for curtain, door and window become the largest and they indeed appear in the area around the red point.}
    \label{33-ranking}
\end{figure}

Therefore, after removing painting, if we want to get clean wall, we still need continue to ablate several top door-, curtain-, window-ACE units, or can also ablating the remaining units with max-activation at the position where other things emerge (Fig. \ref{33-clean}). 
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[t]{1.0in}
    \includegraphics[width=1.0in]{figures/33-ablate_top20.jpg}
    \caption{}
    \label{}
    \end{subfigure}
    \begin{subfigure}[t]{1.0in}
    \includegraphics[width=1.0in]{figures/33-ablate_related.jpg}
    \caption{}
    \label{}
    \end{subfigure}
    \begin{subfigure}[t]{1.0in}
    \includegraphics[width=1.0in]{figures/33-ablate-maxactivation.jpg}
    \caption{}
    \label{}
    \end{subfigure}
    \caption{After ablating top-20 painting-ACE units, we continue to (b) ablate several top door-, curtain-, window-ACE units or (c) ablate remaining units with max activation value at the positions where other things appear and get the image with clean wall at last.}
    \label{33-clean}
\end{figure}
\begin{table}[htbp]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        object & frequency & Average area ratio\\
        \hline\hline
        chair & 75.8\% & 14.95\%\\
        \hline
        table & 69.4\% & 10.16\%\\
        \hline
        person & 28.7\% & 21.01\%\\
        \hline
        painting &  29.0\% & 3.65\%\\
        \hline
        window & 50.7\% & 5.52\%\\
        \hline 
        curtain & 16.7\% & 5.75\%\\
        \hline
        door & 26.8\% & 2.19\%\\
        \hline 
        silver screen & 9.05\% & 2.98\%\\
        \hline
        cabinet & 7.89\% & 2.44\%\\
        \hline
    \end{tabular}
    \caption{The occurrence frequency and average area ratio in the image of different objects in LSUN conference room dataset.}
    \label{LSUN}
\end{table}


Finally, we want to find the causes of different degree of disentangle of different objects. A direct thought is that this is caused by the bias of dataset. Table \ref{LSUN} shows the occurrence frequency and average area ratio in the image of different objects in LSUN conference room dataset.
Compared with other objects, chair and table have higher frequency and relative larger area ratio in the dataset. Therefore, they may be thought by the generator as the inherent attribute of conference room, thus have lower degree of disentangle and many related units with relatively average lower ACE to prevent themselves been removed easily from the images, which improves the robustness of the network. While objects like painting may be thought as variable elements thus have high degree of disentangle and have less, but more influential units with high ACE, which also improves the diversity of the network. And among the objects that would like to appear on the wall (painting, window, curtain, door...), window and door have high frequency. This also explain to some extent that why they are more likely to appear after removing painting from the image and been enhanced by the pixel normalization. 




==> Experiment.tex <==
\section{Experiment}
\subsection{x/x' and $\beta/\beta'$}
In this section, we use a difference-in-difference experiment to reveal the real effect of pixel normalization in image generation of GAN.

We choose layer4 for this and following experiments, because the scale of details in layer4 is suitable for investigating main object classes -- previous layers focus more on the whole scene, lacking enough details, while following layers focus on too small details, such as texture. Then we choose to ablate top-20 causal units, since most main objects in the scene can disappear when we ablate corresponding top-20 causal units (Figure \ref{segarea_ablate20_variousobjects}).

\begin{figure}[htbp]
    \centering
    \includegraphics[width=3.0in]{figures/seg_ablate20.png}
    \caption{To remove a kind of object, we can usually get good result by ablating top-20 units with highest ACE for this objects (e.g. painting, window, light, curtain and person); However, ablating top-20 chair-ACE units only results in a drop of $20\%$ on chairs' area, and we need to ablate at least top-80 chair-ACE units to get a noticeable effect.}
    \label{segarea_ablate20_variousobjects}
\end{figure}

In this experiment, we use a coefficient-fixing generator: when ablating units in layer 4, we keep the pixel normalization coefficients of all layers not changed, as if there were no ablation. In this way, pixel normalization cannot adjust the weights of different units, compared with the original procedure, which increases some units’ weights after ablating others. We also use a units-fixing generator, which does not ablate any units but applies the same pixel normalization coefficients as if we ablated some units. 

For $Y$, we use the original image generated by the conference room generator; for $Y'$, we ablate top-20 chair-causal units in layer 4; for $\underline{Y}$, we apply coefficient-fixing generator and ablate top-20 chair-causal units in layer 4; for $\overline{Y}$, we apply units-fixing generator and set the normalization coefficients as if we ablated top-20 chair-causal units in layer 4. The results are shown in Figure \ref{diff-in-diff}.From the results, we observe that the bright area of (c) is roughly the area of chair class in the original image while the bright area in (a) is around the chairs, such as the area of table class and floor. This indicates the real effect of normalization and ablation separately. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=3.0in]{figures/chair_sc_fix_beta.png}
    \caption{After fixing $\beta$, the drop of chair area is almost proportional to the number of ablated units, which is much better than the case not fix $\beta$.}
    \label{segarea_ablate20}
\end{figure}


\subsection{x/x' and different disentanglement of units}
In this experiment, we mainly study the influence of pixel normalization and ablation on objects with different degree of disentanglement and explain why some other objects will appear after removing certain objects. 

To explain why some objects can be easily removed while others cannot, we first compare the distribution of ACE to chair with that to painting in layer 4. The results are shown below (Figure \ref{ace-distri}). We find that ACE to painting is more concentrated: most units either have great impact on painting class (ACE $\geq$ 0.5) or have a little impact on painting class (ACE around 0.15), while only a few units have ACE in [0.25,0.50). This concentrated distribution is in contrast to the evenly distributed chair-causal units. For chair-causal units, a relatively large proportion of units have ACE in [0.25,0.50), and the proportion of units having ACE around 0.15 is higher than that of painting-causal units. This difference suggests that the painting generation is more specialized than chair generation in layer 4. When we ablate top-20 painting-causal units, most units having great impact on painting class are ablated, and other units only account for a little effect to painting. But when we ablate top-20 chair-causal units, other units still have great impact on chair class. This explains why paintings can be easily removed while chairs cannot.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=3.0in]{figures/distplot.png}
    \caption{The distribution of units from layer 4 over chair-ACE and painting-ACE is shown. A unit is counted if it has ACE $\geq$ 0.15, since we focus on the units with observable effect on chair or painting. Since the units with ACE $\geq$ 0.6 all have great impact on the corresponding object class but are relatively few and distributed, we treat them as units with ACE $=$ 0.6.}
    \label{ace-distri}
\end{figure}
\Li {The text needs modifying.}
Next, we show the degree of disentanglement between different objects based on the former observations, the specialization of units. We investigate the disentanglement between chair and table and between painting and wall by plotting ACE to them of units in layer 4. Since in conference rooms, chairs almost always appear close to the table, and the paintings are always on the wall, the degree of disentanglement of these two groups reflects the easiness of ablating chairs or paintings from the image without affecting the backgrounds. The scatter plots are shown in Figure \ref{scatter-plots}. We also calculate the average ACE to wall of all painting-causal units and the average ACE to table of all chair-causal units.

From the results, we observe that the degree of disentanglement of painting and wall is higher than that of chair and table. So when we ablate painting-causal units, the wall is less affected; when we ablate chair-causal units, the table is more likely to change. Therefore, it is easier to ablate painting class from the image without influencing the wall.


\begin{figure}[htbp]
    \begin{center}
    \begin{subfigure}[t]{2.5in}
    \vspace{0pt}
            \centering\begin{tikzpicture}
            \begin{axis}[
                xlabel={ACE to window},
                ylabel={ACE to wall},
                ylabel absolute, ylabel style={yshift=-0.6cm},
                xlabel absolute, xlabel style={yshift=0.35cm},
                width=6.1cm,
                height=6.1cm,
                label style={font=\tiny},
                ticklabel style={font=\tiny},
                legend style={at={(1,0.35)}, anchor=south east}
            ]
            \pgfplotstableread{data/window-wall.txt}\mydata;
            \addplot[
                scatter,only marks,scatter src=explicit symbolic,
                scatter/classes={
                    2={mark=*,mark size=1,blue}
                }
            ]
            table [x=x,y=y,meta=set]{\mydata};
            % \legend{$\scriptscriptstyle X_1$,$\scriptscriptstyle X_2$,$\scriptscriptstyle X_3$,$\scriptscriptstyle others$}
            \end{axis}
        \end{tikzpicture}
        \centering
    \caption{ACE to window and wall}
    \label{chair-table}
    \end{subfigure}
    \begin{subfigure}[t]{2.5in}
                \vspace{0pt}
                \centering\begin{tikzpicture}
                \begin{axis}[
                    xlabel={ACE to door},
                    ylabel={ACE to wall},
                    ylabel absolute, ylabel style={yshift=-0.6cm},
                    xlabel absolute, xlabel style={yshift=0.35cm},
                    width=6.1cm,
                    height=6.1cm,
                    label style={font=\tiny},
                    ticklabel style={font=\tiny},
                    legend style={at={(1,0.35)}, anchor=south east}
                ]
                \pgfplotstableread{data/door-wall.txt}\mydata;
                \addplot[
                    scatter,only marks,scatter src=explicit symbolic,
                    scatter/classes={
                        2={mark=*,mark size=1,blue}
                    }
                ]
                table [x=x,y=y,meta=set]{\mydata};
                % \legend{$\scriptscriptstyle X_1$,$\scriptscriptstyle X_2$,$\scriptscriptstyle X_3$,$\scriptscriptstyle others$}
                \end{axis}
            \end{tikzpicture}
            \centering
    \caption{ACE to door and wall}
    \label{painting-wall}
    \end{subfigure}
    \caption{The scatter plot of ACE to window and wall of all 512 units and the scatter plot of ACE to door and wall of all 512 units in layer 4. }
    \label{scatter-plots}
    \end{center}
\end{figure}
\jie{@Li chair and painting ACE distribution. Explain why painting can be easily removed.} \Li{Done.}

To explain why other things will appear after removing painting, we first do semantic segmentation on the image after ablating top-20 painting-ACE units. (Figure. \ref{33-seg}) using the same segmenter as GAN Dissecion. The result shows that things that come up are some mixture of window, door, cabinet and fabric similar to curtain. Next, we choose several objects that might appear on the wall and get top-100 units in layer 4 that have the max activation value on the point door appears (Figure \ref{33-ranking}). We calculate and normalize the sum of their ACE for each particular object. We can see before ablation, the ACE for painting is the largest and there are also large ACE for window, curtain, and door, which implies that they are very likely to appear after removing paintings. As expected, after ablating top-20 painting-ACE units, ACE for curtain and door becomes the largest and curtain-like fabric and door indeed appear at this point. Moreover, these remain units' absolute activation value at this point increases by about 9\% because of pixel normalization, which helps the appearance of fabric and door. This shows that GANs generate images by stacking many different features but may only show the most activated feature at last. If we remove some objects with high degree of disentangle, other objects with relatively smaller activated value may appear, and further fill the image under the enhancement of pixel normalization. And if we continue to ablating these remain units with max-activation, we can get clean wall at last (Fig. \ref{33-clean}).

\begin{figure}[htbp]
    \begin{center}
    \begin{subfigure}[t]{0.8in}
    \includegraphics[width=0.8in]{figures/33-original.jpg}
    \label{}
    \setlength{\abovecaptionskip}{0cm}
    \caption{original}
    \end{subfigure}
    \begin{subfigure}[t]{0.8in}
    \includegraphics[width=0.8in]{figures/33-ablate_top20.jpg}
    \label{}
    \setlength{\abovecaptionskip}{0cm}
    \caption{ablate top20}
    \end{subfigure}
    \begin{subfigure}[t]{0.8in}
    \includegraphics[width=0.8in]{figures/33-ablate-seg.png}
    \label{}
    \setlength{\abovecaptionskip}{0cm}
    \caption{Seg1}
    \end{subfigure}
    \begin{subfigure}[t]{0.8in}
    \includegraphics[width=0.8in]{figures/33-segment_of_material.PNG}
    \label{}
    \setlength{\abovecaptionskip}{0cm}
    \caption{Seg2}
    \end{subfigure}
    \hspace{2in}
    \begin{subfigure}[t]{0.8in}
    \includegraphics[width=0.8in]{figures/33-window.PNG}
    \label{}
    \setlength{\abovecaptionskip}{0cm}
    \caption{window}
    \end{subfigure}
    \begin{subfigure}[t]{0.8in}
    \includegraphics[width=0.8in]{figures/33-door.PNG}
    \label{}
    \setlength{\abovecaptionskip}{0cm}
    \caption{door}
    \end{subfigure}
    \begin{subfigure}[t]{0.8in}
    \includegraphics[width=0.8in]{figures/33-cabinet.PNG}
    \label{}
    \setlength{\abovecaptionskip}{0cm}
    \caption{cabinet}
    \end{subfigure}
    \begin{subfigure}[t]{0.8in}
    \includegraphics[width=0.8in]{figures/fabric.PNG}
    \label{}
    \setlength{\abovecaptionskip}{0cm}
    \caption{fabric}
    \end{subfigure}
    \caption{(a) The original picture. (b) After ablating top-20 painting-ACE units in layer 4, the painting totally disappear, but there are some other door-like objects appear. (c)Segmentation of objects. (d)Segmentation of materials. The segmenter thinks the things that come up are some mixture of window, door, cabinet and fabric like curtain.}
    \label{33-seg}
    \end{center}
\end{figure}

Finally, we want to find the causes of different degree of disentangle of different objects. A direct thought is that this is caused by the bias of dataset. Table \ref{LSUN} shows the occurrence frequency and average area ratio in the image of different objects in LSUN conference room dataset.
Compared with other objects, chair and table have higher frequency and relative larger area ratio in the dataset. Therefore, they may be thought by the generator as the inherent attribute of conference room, thus have lower degree of disentangle and many related units with relatively average lower ACE to prevent themselves been removed easily from the images, which improves the robustness of the network. While objects like painting may be thought as variable elements thus have high degree of disentangle and have less, but more influential units with high ACE, which also improves the diversity of the network. And among the objects that would like to appear on the wall (painting, window, curtain, door...), window and door have high frequency. This also explain to some extent that why they are more likely to appear after removing painting from the image and been enhanced by the pixel normalization. 

\begin{table}[htbp]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        object & frequency & Average area ratio\\
        \hline\hline
        chair & 75.8\% & 14.95\%\\
        \hline
        table & 69.4\% & 10.16\%\\
        \hline
        person & 28.7\% & 21.01\%\\
        \hline
        painting &  29.0\% & 3.65\%\\
        \hline
        window & 50.7\% & 5.52\%\\
        \hline 
        curtain & 16.7\% & 5.75\%\\
        \hline
        door & 26.8\% & 2.19\%\\
        \hline 
        silver screen & 9.05\% & 2.98\%\\
        \hline
        cabinet & 7.89\% & 2.44\%\\
        \hline
    \end{tabular}
    \caption{The occurrence frequency and average area ratio in the image of different objects in LSUN conference room dataset.}
    \label{LSUN}
\end{table}

\newpage 

\begin{table}[htbp]
    \centering
    \begin{tabular}{|m{2.0cm}<{\centering}|m{1.8cm}<{\centering}|m{2.4cm}<{\centering}|m{1cm}<{\centering}|m{1cm}<{\centering}|m{1cm}<{\centering}|}
    \hline
    \multicolumn{6}{|c|}{chair}\\
    \hline
    example & ACE rank & ACE distribution & $\underline{Y}-Y$ & $Y'-\overline{Y}$ & $\Delta$ \\
    \hline 
    \includegraphics[width=0.8in]{figures/1-ablate-chair.PNG}
    & 
    \includegraphics[width=0.7in]{figures/1-rank-before.png}
    & 
    \includegraphics[width=0.7in]{figures/chair-ace-distribution.png}
    & 
    \fbox{\includegraphics[width=0.3in]{figures/1-y-yu_1.2.png}}
    &
    \fbox{\includegraphics[width=0.3in]{figures/1-ybar-yprime_0.15.png}}
    &
    \fbox{\includegraphics[width=0.3in]{figures/1-delta_1.1.png}}\\[15pt]
    \hline 
    \multicolumn{6}{|c|}{painting}\\
    \hline
    example &  ACE rank & ACE distribution & $\underline{Y}-Y$ & $Y'-\overline{Y}$ & $\Delta$ \\
    \hline 
    \includegraphics[width=0.8in]{figures/33-ablate-painting.PNG}
    & 
    \includegraphics[width=0.7in]{figures/33-rank-before.png}
    & 
    \includegraphics[width=0.7in]{figures/painting-ace-distribution.png}
    & 
    \fbox{\includegraphics[width=0.3in]{figures/33-y-yu.PNG}}
    &
    \fbox{\includegraphics[width=0.3in]{figures/33-ybar-yprime.PNG}}
    &
    \fbox{\includegraphics[width=0.3in]{figures/33-delta_1.1.png}}\\[15pt]
    \hline 
    
    \multicolumn{6}{|c|}{light}\\
    \hline 
    example & ACE rank & ACE distribution & $\underline{Y}-Y$ & $Y'-\overline{Y}$ & $\Delta$ \\
    \hline
    \includegraphics[width=0.8in]{figures/112-ablate-light.PNG}
    & 
    \includegraphics[width=0.7in]{figures/48-rank_before.png}
    & 
    \includegraphics[width=0.7in]{figures/light-ace-distribution.png}
    & 
    \fbox{\includegraphics[width=0.3in]{figures/112-y-yu0.8.png}}
    &
    \fbox{\includegraphics[width=0.3in]{figures/112-ybar-yprime.PNG}}
    &
    \fbox{\includegraphics[width=0.3in]{figures/112-delta0.8.png}}\\[15pt]
    \hline 
    \end{tabular}
    \caption{experiment summary}
    \label{main_fig}
\end{table}



==> guidance.tex <==
\section{Submission of conference papers to ICLR 2021}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2021 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2021_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2021_conference.sty+ and \verb+iclr2021_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2021_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 8 pages for the main text of the initial submission, with unlimited additional pages for citations. Note that the upper page limit differs from last year!Authors may use as many pages of appendices (after the bibliography) as they wish, but reviewers are not required to read these. During the rebuttal phase and for the camera ready version, authors are allowed one additional page for the main text, for a strict upper limit of 9 pages.

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}




\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

==> related.tex <==
\section{Related Work}
\subsection{Generative Adversarial Network (GAN)}
GAN~\cite{goodfellow2014generative} is a sort of deep learning models with convolutional neural networks (CNN) as the backbone that learns to generate highly realistic images in an unsupervised or self-supervised manner. Early GANs like DCGAN or WGAN trained on simple datasets only generate low resolution images, losing details and diversity of the scenario. Later, sophisticated techniques including normalization and regularization are adopted as modules into larger GAN model such as PG-GAN and BigGAN to generate high fidelity images. 

\subsection{Theoretical analysis on GAN}


\subsection{Experimental analysis on GAN}
